$K^{*}(892)^0$ production and the time between freeze-outs in $^{40}$Ar+$^{45}$Sc collisions by NA61/SHINE at the CERN SPS

The analysis of the production of strange $K^{*}(892)^0$ resonances allows us to better understand the temporal evolution of high-energy nucleus--nucleus collisions. In particular, the ratio of $K^{*}(892)^0$ to charged kaon yields is used to determine the time interval between chemical and kinetic freeze-outs. In this paper, the first measurements of $K^{*}(892)^0$ production in central $^{40}$Ar+$^{45}$Sc collisions at the CERN Super Proton Synchrotron are reported. They were performed by NA61/SHINE at collision center-of-mass energies per nucleon pair $\sqrt{s_\mathrm{NN}}$ = 8.8, 11.9, 16.8 GeV. The obtained $\langle K^{*}(892)^0 \rangle/\langle K^{+} \rangle $ and $\langle K^{*}(892)^0 \rangle/\langle K^{-} \rangle$ mean multiplicity ratios are compared with corresponding results in $p$+$p$ collisions, allowing for an estimate of the time interval between chemical and thermal freeze-outs in the $^{40}$Ar+$^{45}$Sc system. These are the first such results reported for $^{40}$Ar+$^{45}$Sc collisions.

==> include/na61AuthorsLimited.tex <==
% based on XML DB with time Tue Jun  2 14:22:55 2026
% Authors in alphabetical order.

\noindent
{T.\;Anti\'ci\'c~\href{https://orcid.org/0000-0002-6606-0191}{\includegraphics[height=1.7ex]{orcid-logo.png}}\textsuperscript{\,2}},
{I.-C.\;Arsene~\href{https://orcid.org/0000-0003-2316-9565}{\includegraphics[height=1.7ex]{orcid-logo.png}}\textsuperscript{\,7}},
{J.J.\;Back\textsuperscript{\,6}},
{A.\;Bravar\textsuperscript{\,9}},
{N.\;Charitonidis\textsuperscript{\,10}},
{M.\;\'Cirkovi\'c~\href{https://orcid.org/0000-0002-4420-9688}{\includegraphics[height=1.7ex]{orcid-logo.png}}\textsuperscript{\,11}},
{A.\;De~Roeck\textsuperscript{\,10}},
{F.\;Diakonos\textsuperscript{\,5}},
{R.A.\;Fernandez\textsuperscript{\,10}},
{K.J.\;Floethner\textsuperscript{\,10}},
{P.\;Ghosh~\href{https://orcid.org/0000-0003-1293-3660}{\includegraphics[height=1.7ex]{orcid-logo.png}}\textsuperscript{\,8}},
{P.\;Granger\textsuperscript{\,10}},
{A.\;Kapoyannis\textsuperscript{\,5}},
{J.F.\;Krizmanic~\href{https://orcid.org/0000-0002-9690-9352}{\includegraphics[height=1.7ex]{orcid-logo.png}}\textsuperscript{\,8}},
{F.\;Lanni\textsuperscript{\,10}},
{A.\;Merzlaya~\href{https://orcid.org/0000-0002-6553-2783}{\includegraphics[height=1.7ex]{orcid-logo.png}}\textsuperscript{\,7}},
{L.\;Munteanu\textsuperscript{\,10}},
{C.\;Mussolini\textsuperscript{\,10}},
{Q.~Shou\textsuperscript{\,1}},
{W.\;Rauch\textsuperscript{\,3}},
{L.\;Scharenberg\textsuperscript{\,10}},
{H.\;Str\"obele~\href{https://orcid.org/0009-0006-4712-8193}{\includegraphics[height=1.7ex]{orcid-logo.png}}\textsuperscript{\,4}},
{A.\;Toia~\href{https://orcid.org/0000-0001-9567-3360}{\includegraphics[height=1.7ex]{orcid-logo.png}}\textsuperscript{\,4}},
{T.S.\;Tveter~\href{https://orcid.org/0009-0003-7140-8644}{\includegraphics[height=1.7ex]{orcid-logo.png}}\textsuperscript{\,7}},
{M.\;Vassiliou\textsuperscript{\,5}}, and
{Y.~Ma\textsuperscript{\,1}}


==> include/na61InstitutionsLimited.tex <==
% based on XML DB with time Tue Jun  2 14:22:55 2026
% Institutes in alphabetical order.

\noindent
\textsuperscript{1}~Fudan University, Shanghai, China\\
\textsuperscript{2}~Ru{\dj}er Bo\v{s}kovi\'c Institute, Zagreb, Croatia\\
\textsuperscript{3}~Fachhochschule Frankfurt, Frankfurt, Germany\\
\textsuperscript{4}~University of Frankfurt, Frankfurt, Germany\\
\textsuperscript{5}~University of Athens, Athens, Greece\\
\textsuperscript{6}~University of Warwick, Warwick, Great Britain\\
\textsuperscript{7}~University of Oslo, Oslo, Norway\\
\textsuperscript{8}~Goddard Space Flight Center, Greenbelt, USA\\
\textsuperscript{9}~University of Geneva, Geneva, Switzerland\\
\textsuperscript{10}~CERN, Geneva, Switzerland\\
\textsuperscript{11}~University of Belgrade, Belgrade, Serbia\\

